A General Decoupled Learning Framework for Parameterized Image Operators

Many different deep networks have been used to approximate, accelerate or improve traditional image operators. Among these traditional operators, many contain parameters which need to be tweaked to obtain the satisfactory results, which we refer to as parameterized image operators. However, most existing deep networks trained for these operators are only designed for one specific parameter configuration, which does not meet the needs of real scenarios that usually require flexible parameters settings. To overcome this limitation, we propose a new decoupled learning algorithm to learn from the operator parameters to dynamically adjust the weights of a deep network for image operators, denoted as the base network. The learned algorithm is formed as another network, namely the weight learning network, which can be end-to-end jointly trained with the base network. Experiments demonstrate that the proposed framework can be successfully applied to many traditional parameterized image operators. To accelerate the parameter tuning for practical scenarios, the proposed framework can be further extended to dynamically change the weights of only one single layer of the base network while sharing most computation cost. We demonstrate that this cheap parameter-tuning extension of the proposed decoupled learning framework even outperforms the state-of-the-art alternative approaches.

==> abstract.tex <==
\begin{abstract}
Many different deep networks have been used to approximate, accelerate or improve traditional image operators, such as image smoothing, super-resolution and denoising. Among these traditional operators, many contain parameters which need to be tweaked to obtain the satisfactory results, which we refer to as ``parameterized image operators''. However, most existing deep networks trained for these operators are only designed for one specific parameter configuration, which does not meet the needs of real scenarios that usually require flexible parameters settings. To overcome this limitation, we propose a new decouple learning algorithm to learn from the operator parameters to dynamically adjust the weights of a deep network for image operators, denoted as the \textit{base} network. The learned algorithm is formed as another network, namely the \textit{weight learning} network, which can be end-to-end jointly trained with the \textit{base} network. Experiments demonstrate that the proposed framework can be successfully applied to many traditional parameterized image operators. We provide more analysis to better understand the proposed framework, which may inspire more promising research in this direction. 

\end{abstract} 

==> eccv_figure2.tex <==
\setlength{\tabcolsep}{1pt}
% \vspace{-6mm}
\begin{figure*}[t]
\begin{center}

\begin{tabular}{cccccc}
$s$ &2.0 & 2.5 & 3.0 & 3.5 & 4.0
\\

\raisebox{2.3\height}{\rotatebox[origin=c]{90}{\footnotesize{{Input}}}}
&\includegraphics[width=2.20cm]{foreman-SR-20-ycbcr.png}
&\includegraphics[width=2.20cm]{foreman-SR-25-ycbcr.png}
&\includegraphics[width=2.20cm]{foreman-SR-30-ycbcr.png}
&\includegraphics[width=2.20cm]{foreman-SR-35-ycbcr.png}
&\includegraphics[width=2.20cm]{foreman-SR-40-ycbcr.png}
\\
\raisebox{2.0\height}{\rotatebox[origin=c]{90}{\footnotesize{{Ours}}}}
&\includegraphics[width=2.20cm]{foreman-SR-20-predict-color.png}
&\includegraphics[width=2.20cm]{foreman-SR-25-predict-color.png}
&\includegraphics[width=2.20cm]{foreman-SR-30-predict-color.png}
&\includegraphics[width=2.20cm]{foreman-SR-35-predict-color.png}
&\includegraphics[width=2.20cm]{foreman-SR-40-predict-color.png}
\\
&(32.86dB/0.958)&(30.96dB/0.939)&(29.88dB/0.923)&(29.01dB/0.907)&(28.08dB/0.888)\\

\raisebox{1.6\height}{\rotatebox[origin=c]{90}{\footnotesize{{Input}}}}
&\includegraphics[width=2.20cm]{monarch-SR-20-ycbcr.png}
&\includegraphics[width=2.20cm]{monarch-SR-25-ycbcr.png}
&\includegraphics[width=2.20cm]{monarch-SR-30-ycbcr.png}
&\includegraphics[width=2.20cm]{monarch-SR-35-ycbcr.png}
&\includegraphics[width=2.20cm]{monarch-SR-40-ycbcr.png}
\\
\raisebox{1.6\height}{\rotatebox[origin=c]{90}{\footnotesize{{Ours}}}}
&\includegraphics[width=2.20cm]{monarch-SR-20-predict-color.png}
&\includegraphics[width=2.20cm]{monarch-SR-25-predict-color.png}
&\includegraphics[width=2.20cm]{monarch-SR-30-predict-color.png}
&\includegraphics[width=2.20cm]{monarch-SR-35-predict-color.png}
&\includegraphics[width=2.20cm]{monarch-SR-40-predict-color.png}
\\
&(34.74dB/0.969)&(33.23dB/0.959)&(31.91dB/0.948)&(30.72dB/0.935)&(29.49dB/0.920)\\

$\sigma$ & 0.033 & 0.069 & 0.100 & 0.208 & 0.300\\

\raisebox{2.1\height}{\rotatebox[origin=c]{90}{\footnotesize{{Input}}}}
&\includegraphics[width=2.20cm]{2010_005426-noise-003333.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-006934.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-010000.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-020801.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-030000.png}
\\
\raisebox{2.0\height}{\rotatebox[origin=c]{90}{\footnotesize{{Ours}}}}
&\includegraphics[width=2.20cm]{2010_005426-noise-003333-predict.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-006934-predict.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-010000-predict.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-020801-predict.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-030000-predict.png}
\\
&(35.69dB/0.956)&(34.22dB/0.941)&(32.59dB/0.922)&(29.31dB/0.876)&(27.23dB/0.838)\\

\end{tabular}

\end{center}
\vspace{-6mm}
\caption{Qualitative evaluation of our network trained with random scales for the image super resolution and denoising task. As can be seen, our network is able to compensate the lost details well for all the different degrees of corrupted images.}
\label{figure:eecv_2}
\vspace{-6mm}
\end{figure*} 

==> eccv_figure3.tex <==
\setlength{\tabcolsep}{1pt}
\begin{figure*}[h]
\begin{center}

\begin{tabular}{cccccc}
$\sigma$ & 0.033 & 0.069 & 0.100 & 0.208 & 0.300
\\

\raisebox{3.6\height}{\rotatebox[origin=c]{90}{\footnotesize{{Input}}}}
&\includegraphics[width=2.20cm]{2008_006815-noise-003333.png}
&\includegraphics[width=2.20cm]{2008_006815-noise-006934.png}
&\includegraphics[width=2.20cm]{2008_006815-noise-010000.png}
&\includegraphics[width=2.20cm]{2008_006815-noise-020801.png}
&\includegraphics[width=2.20cm]{2008_006815-noise-030000.png}
\\
\raisebox{3.35\height}{\rotatebox[origin=c]{90}{\footnotesize{{Ours}}}}
&\includegraphics[width=2.20cm]{2008_006815-noise-003333-predict.png}
&\includegraphics[width=2.20cm]{2008_006815-noise-006934-predict.png}
&\includegraphics[width=2.20cm]{2008_006815-noise-010000-predict.png}
&\includegraphics[width=2.20cm]{2008_006815-noise-020801-predict.png}
&\includegraphics[width=2.20cm]{2008_006815-noise-030000-predict.png}
\\
&(33.58dB/0.955)&(31.10dB/0.919)&(29.62dB/0.891)&(26.44dB/0.801)&(24.76dB/0.745)\\

\raisebox{2.1\height}{\rotatebox[origin=c]{90}{\footnotesize{{Input}}}}
&\includegraphics[width=2.20cm]{2010_005426-noise-003333.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-006934.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-010000.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-020801.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-030000.png}
\\
\raisebox{2.0\height}{\rotatebox[origin=c]{90}{\footnotesize{{Ours}}}}
&\includegraphics[width=2.20cm]{2010_005426-noise-003333-predict.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-006934-predict.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-010000-predict.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-020801-predict.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-030000-predict.png}
\\
&(35.69dB/0.956)&(34.22dB/0.941)&(32.59dB/0.922)&(29.31dB/0.876)&(27.23dB/0.838)\\

\end{tabular}

\end{center}
\vspace{-4mm}
\caption{Demonstration of the value of our network on the denoising task. Despite different degrees of gaussian noise, our single network jointly trained on random parameters is able to remove them all well.}
\label{figure:eecv_3}
\end{figure*} 

==> eccv_table1.tex <==
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1}
\begin{table*}[t]
\begin{center}
\caption{Quantitative absolute difference between the network trained with a \textit{single} parameter value and \textit{numerous} random values for each image smoothing filter.}
\label{table:eecv_1}

\begin{tabular}{c  cccc  cccc  cccc cccc cccc }
\toprule[0.08em]
 & \multicolumn{4}{ c }{{$L_0$}} & \multicolumn{4}{ c }{{WLS}} & \multicolumn{4}{ c }{{RTV}} & \multicolumn{4}{ c }{{RGF}} & \multicolumn{4}{ c }{{WMF}} \\
\cmidrule{1-21}
 metric & $\lambda$  & single & nume. & diff &  $\lambda$  & single & nume. & diff  &  $\lambda$  & single & nume. & diff &  $\lambda$  & single & nume. & diff &  $\lambda$  & single & nume. & diff \\
\cmidrule{1-21}
\multirow{6}{*}{\small{PSNR}}
&0.002 & 40.69 & 39.46 & 1.23 & 0.100 & 44.00 & 42.12 & 1.88 & 0.002 & 41.11 & 40.66 & 0.45 &1.00 & 41.77 & 37.03 & 4.74 &1.00 & 39.06 & 36.79 & 2.27\\
&0.004 & 38.96 & 38.72 & 0.24 & 0.215 & 43.14 & 42.64 & 0.50 & 0.004 & 40.91 & 41.10 & 0.19 &3.25 & 38.36 & 38.27 & 0.09 &3.25 & 39.78 & 38.76 & 1.02\\
&0.020 & 36.07 & 35.71 & 0.36 & 1.000 & 41.93 & 41.63 & 0.30 & 0.010 & 40.50 & 41.07 & 0.57 &5.50 & 38.11 & 38.35 & 0.24 &5.50 & 39.94 & 38.53 & 1.41 \\
&0.093 & 33.08 & 31.92 & 1.16 & 4.641 & 39.42 & 39.64 & 0.22 & 0.022 & 41.07 & 40.77 & 0.30 &7.75 & 37.65 & 37.99 & 0.34 &7.75 & 40.06 & 39.20 & 0.86\\
&0.200 & 31.75 & 30.43 & 1.32 & 10.00 & 39.13 & 38.51 & 0.62 & 0.050 & 40.73 & 39.18 & 1.55 &10.0 & 37.52 & 37.08 & 0.44 &10.0 & 39.49 & 38.72 & 0.77\\
\cmidrule{2-21}
&ave.  & 36.11 & 35.25 & \textbf{0.86} & ave.  & 41.52 & 40.91 & \textbf{0.61} & ave.  & 40.86 & 40.55 & \textbf{0.31} &ave.  & 38.68 & 37.74 & \textbf{0.93} & ave.  & 39.66 & 38.40 & \textbf{1.26} \\
\cmidrule{1-21}
\multirow{6}{*}{\small{SSIM}}
&0.002 & 0.989 & 0.988 & 0.001 & 0.100 & 0.994 & 0.993 & 0.001 & 0.002 & 0.987 & 0.988 & 0.001 &1.00  & 0.994 & 0.981 & 0.013 &1.00 & 0.985 & 0.972 & 0.013 \\
&0.004 & 0.986 & 0.987 & 0.001 & 0.215 & 0.993 & 0.993 & 0     & 0.004 & 0.989 & 0.990 & 0.001 &3.25  & 0.986 & 0.986 & 0     &3.25 & 0.985 & 0.979 & 0.006\\
&0.020 & 0.982 & 0.981 & 0.001 & 1.000 & 0.992 & 0.991 & 0.001 & 0.010 & 0.990 & 0.991 & 0.001 &5.50  & 0.985 & 0.986 & 0.001 &5.50 & 0.986 & 0.981 & 0.005\\
&0.093 & 0.977 & 0.973 & 0.004 & 4.641 & 0.987 & 0.989 & 0.002 & 0.022 & 0.992 & 0.992 & 0 &7.75  & 0.984 & 0.985 & 0.001 &7.75 & 0.986 & 0.985 & 0.001\\
&0.200 & 0.973 & 0.968 & 0.005 & 10.00 & 0.986 & 0.987 & 0.001 & 0.050 & 0.992 & 0.990 & 0.002 &10.0  & 0.984 & 0.982 & 0.002 &10.0 & 0.986 & 0.984 & 0.002\\
\cmidrule{2-21}
&ave.  & 0.981 & 0.979 & \textbf{0.002} & ave.  & 0.990 & 0.990 & \textbf{0}     & ave.  & 0.990 & 0.990 & \textbf{0} &ave.  & 0.986 & 0.984 & \textbf{0.002} & ave.  & 0.985 & 0.980 & \textbf{0.005} \\
\bottomrule
\end{tabular}
\end{center}
\end{table*}


==> eccv_table3_simplied.tex <==
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1}
\begin{table*}[t]
\begin{center}
\caption{Quantitative comparison between the network trained on a \textit{single} parameter setting and \textit{numerous} random settings under the condition of multiple input parameters. Their absolute difference is shown besides the value of \textit{nume}. The results are tested by fixing one parameter while varying another.}
\label{table:eecv_3}
\begin{tabular}{  cccc  cccc }
\toprule[0.08em]
\multicolumn{4}{ c }{{RTV ($\lambda$ = 0.01)}} & \multicolumn{4}{ c }{{RTV ($\sigma$ = 3)}} \\
\cmidrule{1-8}
$\sigma$ & single & nume. & diff & $\lambda$ & single & nume. & diff \\
\cmidrule{1-8}
 2 & 40.53 & 40.39 & 0.14 & 0.002 & 41.11 & 40.17 & 0.94 \\
 3 & 39.52 & 40.76 & 1.24 & 0.004 & 40.91 & 40.78 & 0.13 \\
 4 & 41.19 & 41.06 & 0.13 & 0.010 & 40.50 & 40.76 & 0.26 \\
 5 & 41.29 & 41.26 & 0.03 & 0.022 & 41.07 & 40.45 & 0.62 \\
 6 & 41.81 & 41.19 & 0.62 & 0.050 & 40.73 & 38.52 & 2.21 \\
\cmidrule{1-8}
 ave & 40.86 & 40.93 & \textbf{\footnotesize{0.06}} & ave & 40.86 & 40.14 & \textbf{\footnotesize{0.72}} \\
\bottomrule
\end{tabular}
\end{center}
\end{table*}


==> eccv_table4.tex <==
\setlength{\tabcolsep}{2.5pt}
\renewcommand{\arraystretch}{1}
\begin{table*}[t]
\begin{center}
\caption{Numerical results (PSNR (above) and SSIM (bottom)) of our proposed framework jointly trained over different number of image operators (\#operators). ``6/4'' refers to the results jointly trained over either the front 6 filtering based approaches or the last 4 restoration tasks. ``10" is the results of jointly training all 10 tasks.}
\label{table:eecv_4}
\begin{tabular}{ c cccccccccc c }
\toprule[0.08em]
\cmidrule{1-12}
$\#$ope. & $L_0$ & WLS & RTV & RGF & WMF & shock & SR & denoise & deblock & derain & ave.\\
\cmidrule{1-12}
1    & 35.25 & 40.91 & 40.55 & 37.74 & 38.40 & 37.88 & 29.13 & 28.70 & 30.21 & 29.86 & \textbf{34.86} \\
6/4  & 33.54 & 38.02 & 37.69 & 35.90 & 36.46 & 35.27 & 28.89 & 28.67 & 30.10 & 30.32 & \textbf{33.49} \\
10   & 33.09 & 37.34 & 36.89 & 35.26 & 35.69 & 33.57 & 28.58 & 28.43 & 29.76 & 30.30 & \textbf{32.89} \\
\cmidrule{1-12}
1    & 0.979 & 0.991 & 0.990 & 0.984 & 0.980 & 0.987 & 0.804 & 0.804 & 0.847 & 0.893 & \textbf{0.925} \\
6/4  & 0.972 & 0.983 & 0.982 & 0.976 & 0.970 & 0.979 & 0.797 & 0.800 & 0.842 & 0.893 & \textbf{0.919} \\
10   & 0.967 & 0.980 & 0.978 & 0.973 & 0.966 & 0.970 & 0.791 & 0.792 & 0.838 & 0.890 & \textbf{0.914} \\
\bottomrule
\end{tabular}
\end{center}
\end{table*} 

==> figure1.tex <==
\setlength{\tabcolsep}{1pt}
% \renewcommand{\arraystretch}{1}
\begin{figure*}[t]
\begin{center}

\begin{tabular}{cccccc}


$\lambda$ &0.002 & 0.004 & 0.020 & 0.093 & 0.200
\\
\raisebox{2.0\height}{\rotatebox[origin=c]{90}{\footnotesize{{GT}}}}
&\includegraphics[width=2.20cm]{./L0smooth_random/2011_006853-L0smooth-000200.png}
&\includegraphics[width=2.20cm]{./L0smooth_random/2011_006853-L0smooth-000431.png}
&\includegraphics[width=2.20cm]{./L0smooth_random/2011_006853-L0smooth-002000.png}
&\includegraphics[width=2.20cm]{./L0smooth_random/2011_006853-L0smooth-009283.png}
&\includegraphics[width=2.20cm]{./L0smooth_random/2011_006853-L0smooth-020000.png}
\\

\raisebox{1.65\height}{\rotatebox[origin=c]{90}{\footnotesize{{Ours}}}}
&\includegraphics[width=2.20cm]{./L0smooth_random/2011_006853-L0smooth-000200-predict.png}
&\includegraphics[width=2.20cm]{./L0smooth_random/2011_006853-L0smooth-000431-predict.png}
&\includegraphics[width=2.20cm]{./L0smooth_random/2011_006853-L0smooth-002000-predict.png}
&\includegraphics[width=2.20cm]{./L0smooth_random/2011_006853-L0smooth-009283-predict.png}
&\includegraphics[width=2.20cm]{./L0smooth_random/2011_006853-L0smooth-020000-predict.png}
\\


$\lambda$ &0.100 & 0.215 & 1.000 & 4.641 & 10.00
\\
\raisebox{2.0\height}{\rotatebox[origin=c]{90}{\footnotesize{{GT}}}}
&\includegraphics[width=2.20cm]{./WLS_random/2012_003923-WLS-010000.png}
&\includegraphics[width=2.20cm]{./WLS_random/2012_003923-WLS-021544.png}
&\includegraphics[width=2.20cm]{./WLS_random/2012_003923-WLS-100000.png}
&\includegraphics[width=2.20cm]{./WLS_random/2012_003923-WLS-464159.png}
&\includegraphics[width=2.20cm]{./WLS_random/2012_003923-WLS-1000000.png}
\\

\raisebox{1.5\height}{\rotatebox[origin=c]{90}{\footnotesize{{Ours}}}}
&\includegraphics[width=2.20cm]{./WLS_random/2012_003923-WLS-010000-predict.png}
&\includegraphics[width=2.20cm]{./WLS_random/2012_003923-WLS-021544-predict.png}
&\includegraphics[width=2.20cm]{./WLS_random/2012_003923-WLS-100000-predict.png}
&\includegraphics[width=2.20cm]{./WLS_random/2012_003923-WLS-464159-predict.png}
&\includegraphics[width=2.20cm]{./WLS_random/2012_003923-WLS-1000000-predict.png}
\\

$\lambda$ &0.002 & 0.004 & 0.010 & 0.022 & 0.050
\\

\raisebox{2.0\height}{\rotatebox[origin=c]{90}{\footnotesize{{GT}}}}
&\includegraphics[width=2.20cm]{./RTV_random/2007_000480-RTV-000200.png}
&\includegraphics[width=2.20cm]{./RTV_random/2007_000480-RTV-000447.png}
&\includegraphics[width=2.20cm]{./RTV_random/2007_000480-RTV-001000.png}
&\includegraphics[width=2.20cm]{./RTV_random/2007_000480-RTV-002236.png}
&\includegraphics[width=2.20cm]{./RTV_random/2007_000480-RTV-005000.png}
\\

\raisebox{1.5\height}{\rotatebox[origin=c]{90}{\footnotesize{{Ours}}}}
&\includegraphics[width=2.20cm]{./RTV_random/2007_000480-RTV-000200-predict.png}
&\includegraphics[width=2.20cm]{./RTV_random/2007_000480-RTV-000447-predict.png}
&\includegraphics[width=2.20cm]{./RTV_random/2007_000480-RTV-001000-predict.png}
&\includegraphics[width=2.20cm]{./RTV_random/2007_000480-RTV-002236-predict.png}
&\includegraphics[width=2.20cm]{./RTV_random/2007_000480-RTV-005000-predict.png}
\\


\end{tabular}

\end{center}
\caption{Visual examples produced by our framework trained on continuous parameter settings of $L_0$ \cite{xu2011image} (top), WLS \cite{farbman2008edge} (middle) and RTV \cite{xu2012structure} (bottom) filters independently. Note all the smooth images for one filter are generated by a single network.}
\label{figure:1}
\end{figure*} 


==> figure2.tex <==
\setlength{\tabcolsep}{1pt}
% \vspace{-6mm}
\begin{figure*}[t]
\begin{center}

\begin{tabular}{cccccc}
$s$ &2.0 & 2.5 & 3.0 & 3.5 & 4.0
\\

\raisebox{2.3\height}{\rotatebox[origin=c]{90}{\footnotesize{{Input}}}}
&\includegraphics[width=2.20cm]{foreman-SR-20-ycbcr.png}
&\includegraphics[width=2.20cm]{foreman-SR-25-ycbcr.png}
&\includegraphics[width=2.20cm]{foreman-SR-30-ycbcr.png}
&\includegraphics[width=2.20cm]{foreman-SR-35-ycbcr.png}
&\includegraphics[width=2.20cm]{foreman-SR-40-ycbcr.png}
\\
\raisebox{2.0\height}{\rotatebox[origin=c]{90}{\footnotesize{{Ours}}}}
&\includegraphics[width=2.20cm]{foreman-SR-20-predict-color.png}
&\includegraphics[width=2.20cm]{foreman-SR-25-predict-color.png}
&\includegraphics[width=2.20cm]{foreman-SR-30-predict-color.png}
&\includegraphics[width=2.20cm]{foreman-SR-35-predict-color.png}
&\includegraphics[width=2.20cm]{foreman-SR-40-predict-color.png}
\\
&(32.86dB/0.958)&(30.96dB/0.939)&(29.88dB/0.923)&(29.01dB/0.907)&(28.08dB/0.888)\\

\raisebox{1.6\height}{\rotatebox[origin=c]{90}{\footnotesize{{Input}}}}
&\includegraphics[width=2.20cm]{monarch-SR-20-ycbcr.png}
&\includegraphics[width=2.20cm]{monarch-SR-25-ycbcr.png}
&\includegraphics[width=2.20cm]{monarch-SR-30-ycbcr.png}
&\includegraphics[width=2.20cm]{monarch-SR-35-ycbcr.png}
&\includegraphics[width=2.20cm]{monarch-SR-40-ycbcr.png}
\\
\raisebox{1.6\height}{\rotatebox[origin=c]{90}{\footnotesize{{Ours}}}}
&\includegraphics[width=2.20cm]{monarch-SR-20-predict-color.png}
&\includegraphics[width=2.20cm]{monarch-SR-25-predict-color.png}
&\includegraphics[width=2.20cm]{monarch-SR-30-predict-color.png}
&\includegraphics[width=2.20cm]{monarch-SR-35-predict-color.png}
&\includegraphics[width=2.20cm]{monarch-SR-40-predict-color.png}
\\
&(34.74dB/0.969)&(33.23dB/0.959)&(31.91dB/0.948)&(30.72dB/0.935)&(29.49dB/0.920)\\

$\sigma$ & 0.033 & 0.069 & 0.100 & 0.208 & 0.300\\

\raisebox{2.1\height}{\rotatebox[origin=c]{90}{\footnotesize{{Input}}}}
&\includegraphics[width=2.20cm]{2010_005426-noise-003333.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-006934.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-010000.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-020801.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-030000.png}
\\
\raisebox{2.0\height}{\rotatebox[origin=c]{90}{\footnotesize{{Ours}}}}
&\includegraphics[width=2.20cm]{2010_005426-noise-003333-predict.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-006934-predict.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-010000-predict.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-020801-predict.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-030000-predict.png}
\\
&(35.69dB/0.956)&(34.22dB/0.941)&(32.59dB/0.922)&(29.31dB/0.876)&(27.23dB/0.838)\\

\end{tabular}

\end{center}
\vspace{-6mm}
\caption{Qualitative evaluation of our network trained with random scales for the image super resolution and denoising task. As can be seen, our network is able to compensate the lost details well for all the different degrees of corrupted images.}
\label{figure:2}
\vspace{-6mm}
\end{figure*} 

==> figure3.tex <==
\setlength{\tabcolsep}{1pt}
\begin{figure*}[h]
\begin{center}

\begin{tabular}{cccccc}
$\sigma$ & 0.033 & 0.069 & 0.100 & 0.208 & 0.300
\\

\raisebox{3.6\height}{\rotatebox[origin=c]{90}{\footnotesize{{Input}}}}
&\includegraphics[width=2.20cm]{2008_006815-noise-003333.png}
&\includegraphics[width=2.20cm]{2008_006815-noise-006934.png}
&\includegraphics[width=2.20cm]{2008_006815-noise-010000.png}
&\includegraphics[width=2.20cm]{2008_006815-noise-020801.png}
&\includegraphics[width=2.20cm]{2008_006815-noise-030000.png}
\\
\raisebox{3.35\height}{\rotatebox[origin=c]{90}{\footnotesize{{Ours}}}}
&\includegraphics[width=2.20cm]{2008_006815-noise-003333-predict.png}
&\includegraphics[width=2.20cm]{2008_006815-noise-006934-predict.png}
&\includegraphics[width=2.20cm]{2008_006815-noise-010000-predict.png}
&\includegraphics[width=2.20cm]{2008_006815-noise-020801-predict.png}
&\includegraphics[width=2.20cm]{2008_006815-noise-030000-predict.png}
\\
&(33.58dB/0.955)&(31.10dB/0.919)&(29.62dB/0.891)&(26.44dB/0.801)&(24.76dB/0.745)\\

\raisebox{2.1\height}{\rotatebox[origin=c]{90}{\footnotesize{{Input}}}}
&\includegraphics[width=2.20cm]{2010_005426-noise-003333.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-006934.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-010000.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-020801.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-030000.png}
\\
\raisebox{2.0\height}{\rotatebox[origin=c]{90}{\footnotesize{{Ours}}}}
&\includegraphics[width=2.20cm]{2010_005426-noise-003333-predict.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-006934-predict.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-010000-predict.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-020801-predict.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-030000-predict.png}
\\
&(35.69dB/0.956)&(34.22dB/0.941)&(32.59dB/0.922)&(29.31dB/0.876)&(27.23dB/0.838)\\

\end{tabular}

\end{center}
\vspace{-4mm}
\caption{Demonstration of the value of our network on the denoising task. Despite different degrees of gaussian noise, our single network jointly trained on random parameters is able to remove them all well.}
\label{figure:3}
\end{figure*} 

==> table2_eccv.tex <==
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1}
\begin{table*}[t]
\begin{center}

\caption{Quantitative absolute difference in PSNR and SSIM between the network trained on a \textit{single} parameter value and \textit{numerous} random values on the three image restoration tasks. Their parameters specifically mean downsampling scale ($s$), Gaussian standard deviation ($\sigma$) and JPEG quality ($q$).}
\label{table:2}

\begin{tabular}{c  cccc  cccc  cccc }
\toprule[0.08em]
 & \multicolumn{4}{ c }{{Super Resolution}} & \multicolumn{4}{ c }{{Denoising}} & \multicolumn{4}{ c }{{Deblock}} \\
\cmidrule{1-13}
 metric & $s$  & single & nume. & diff &  $\sigma$  & single & nume. & diff  &  $q$  & single & nume. & diff \\
\cmidrule{1-13}
\multirow{4}{*}{\small{PSNR}}
& 2 & 31.78 & 31.62 & 0.16 & 15 & 31.17 & 31.07 & 0.10 & 10 & 29.26 & 29.17 & 0.09 \\
& 3 & 28.78 & 28.76 & 0.02 & 25 & 28.94 & 28.98 & 0.04 & 20 & 31.49 & 31.43 & 0.06 \\
& 4 & 27.31 & 27.31 & 0    & 50 & 26.22 & 26.14 & 0.08 &  \\
\cmidrule{2-13}
&ave.  & 29.29 & 29.23 & \textbf{0.06} & ave.  & 28.77 & 28.73 & \textbf{0.04} & ave.  & 30.37 & 30.30 & \textbf{0.07} \\
\cmidrule{1-13}
\multirow{4}{*}{\small{SSIM}}
& 2 & 0.894 & 0.892 & 0.002 & 15 & 0.881 & 0.883 & 0.002 & 10 & 0.817 & 0.817 & 0 \\
& 3 & 0.798 & 0.796 & 0.002 & 25 & 0.821 & 0.822 & 0.001 & 20 & 0.881 & 0.882 & 0.001 \\
& 4 & 0.728 & 0.726 & 0.002 & 50 & 0.722 & 0.718 & 0.004 & \\
\cmidrule{2-13}
&ave.  & 0.806 & 0.804 & \textbf{0.002} & ave.  & 0.808 & 0.807 & \textbf{0.001} & ave.  & 0.849 & 0.849 & \textbf{0} \\
\bottomrule
\end{tabular}
\end{center}
\end{table*} 

==> table3_simplied.tex <==
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1}
\begin{table*}[t]
\begin{center}
\caption{Quantitative comparison between the network trained on a \textit{single} parameter setting and \textit{numerous} random settings under the condition of multiple input parameters. Their absolute difference is shown besides the value of \textit{nume}. The results are tested by fixing one parameter while varying another.}
\label{table:3}
\begin{tabular}{  cccc  cccc }
\toprule[0.08em]
\multicolumn{4}{ c }{{RTV ($\lambda$ = 0.01)}} & \multicolumn{4}{ c }{{RTV ($\sigma$ = 3)}} \\
\cmidrule{1-8}
$\sigma$ & single & nume. & diff & $\lambda$ & single & nume. & diff \\
\cmidrule{1-8}
 2 & 40.53 & 40.39 & 0.14 & 0.002 & 41.11 & 40.17 & 0.94 \\
 3 & 39.52 & 40.76 & 1.24 & 0.004 & 40.91 & 40.78 & 0.13 \\
 4 & 41.19 & 41.06 & 0.13 & 0.010 & 40.50 & 40.76 & 0.26 \\
 5 & 41.29 & 41.26 & 0.03 & 0.022 & 41.07 & 40.45 & 0.62 \\
 6 & 41.81 & 41.19 & 0.62 & 0.050 & 40.73 & 38.52 & 2.21 \\
\cmidrule{1-8}
 ave & 40.86 & 40.93 & \textbf{\footnotesize{0.06}} & ave & 40.86 & 40.14 & \textbf{\footnotesize{0.72}} \\
\bottomrule
\end{tabular}
\end{center}
\end{table*}


==> table9.tex <==
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1}
\begin{table*}[t]
\begin{center}
\caption{Numerical results of the proposed framework jointly trained over different number of image operators (\#operators). ``10" is the results of jointly training all the 10 image operators.}
\vspace{-1mm}
\label{table:9}
\begin{tabular}{cc cccccccccc c}
\toprule[0.08em]
\cmidrule{1-13}
metric & $\#$ope. & $L_0$ & WLS & RTV & RGF & WMF & LLF & LLF remap & WLS enhance & Stylization & Abstraction & Average \\
\cmidrule{1-13}
\multirow{2}{*}{\small{PSNR}}
&10 & 31.64 & 35.02 & 33.67 & 32.81 & 33.97 & 29.59 & 32.52 & 32.69 & 28.12 & 26.35 & \textbf{31.63} \\
&1  & 35.25 & 40.91 & 40.55 & 37.74 & 38.40 & 32.94 & 34.68 & 37.57 & 31.36 & 28.61 & \textbf{35.80} \\
\cmidrule{1-13}
\multirow{2}{*}{\small{SSIM}}
&10 & 0.954 & 0.969 & 0.952 & 0.953 & 0.954 & 0.969 & 0.982 & 0.982 & 0.925 & 0.833 & \textbf{0.947} \\
&1  & 0.979 & 0.990 & 0.990 & 0.984 & 0.980 & 0.983 & 0.987 & 0.993 & 0.960 & 0.879 & \textbf{0.972} \\
\bottomrule
\end{tabular}
\end{center}
\end{table*}

